ILC Reference Design Report Volume 1 - Executive Summary

The International Linear Collider (ILC) is a 200-500 GeV center-of-mass high-luminosity linear electron-positron collider, based on 1.3 GHz superconducting radio-frequency (SCRF) accelerating cavities. The ILC has a total footprint of about 31 km and is designed for a peak luminosity of 2x10^34 cm^-2s^-1. This report is the Executive Summary (Volume I) of the four volume Reference Design Report. It gives an overview of the physics at the ILC, the accelerator design and value estimate, the detector concepts, and the next steps towards project realization.

==> orig/ILC-ES.tex <==
\clearpage
\input{resetcounters}

\chapter{Physics Case for a Terascale e$^+$e$^-$ Linear Collider}

\input{PhysCase}

\clearpage

\input{resetcounters}

\chapter{The ILC Accelerator}\label{chapAcc}

The ILC is
based on 1.3 GHz superconducting radio-frequency (SCRF) accelerating
cavities. The use of the SCRF technology was recommended by
the International Technology Recommendation Panel (ITRP) in August
2004 [M1], and shortly thereafter endorsed by the International
Committee for Future Accelerators (ICFA). In an unprecedented
milestone in high-energy physics, the many institutes around the world
involved in linear collider R\&D united in a common effort to produce a
global design for the ILC.  In November 2004, the 1st International
Linear Collider Workshop was held at KEK, Tsukuba, Japan. The workshop
was attended by some 200 physicists and engineers from around the world,
and paved the way for the 2nd ILC Workshop in August 2005, held at
Snowmass, Colorado, USA, where the ILC Global Design Effort (GDE) was
officially formed. The GDE membership reflects the global nature of
the collaboration, with accelerator experts from all three regions
(Americas, Asia and Europe). The first major goal of the GDE was to
define the basic parameters and layout of the machine -- the Baseline
Configuration. This was achieved at the first GDE meeting held at
INFN, Frascati, Italy in December 2005 with the creation of the
Baseline Configuration Document (BCD). During the next 14 months, the
BCD was used as the basis for the detailed design work and value
estimate (as described in section 1.6) culminating in the completion
of the second major milestone, the publication of the draft ILC
Reference Design Report (RDR).


The technical design and cost estimate for the ILC is based on two
decades of world-wide Linear Collider R\&D, beginning with the
construction and operation of the SLAC Linear Collider (SLC). The SLC
is acknowledged as a proof-of-principle machine for the linear
collider concept. The ILC SCRF linac technology was pioneered by the
TESLA collaboration\footnote{Now known as the TESLA Technology
  Collaboration (TTC); see http://tesla.desy/de/ .}, culminating in a
proposal for a 500 GeV center-of-mass linear collider in
2001~\cite{tdr}. The concurrent (competing) design work on a normal
conducting collider (NLC with X-band~\cite{nlc} and GLC with X- or
C-Band~\cite{glc}), has advanced the design concepts for the ILC
injectors, Damping Rings (DR) and Beam Delivery System (BDS), as well
as addressing overall operations, machine protection and availability
issues. The X- and C-band R\&D has led to concepts for RF power
sources that may eventually produce either cost and/or performance
benefits. Finally, the European XFEL [M5] to be constructed at DESY,
Hamburg, Germany, will make use of the TESLA linac technology, and
represents a significant on-going R\&D effort of great
benefit for the ILC.

The current ILC baseline assumes an average accelerating gradient of
31.5 MV/m in the cavities to achieve a center-of-mass energy of 500
GeV. The high luminosity requires the use of high power and small
emittance beams. The choice of 1.3 GHz SCRF is well suited to the
requirements, primarily because the very low power loss in the SCRF
cavity walls allows the use of long RF pulses, relaxing the
requirements on the peak-power generation, and ultimately leading to
high wall-plug to beam transfer efficiency.

The primary cost drivers are the SCRF Main Linac technology and the
Conventional Facilities (including civil engineering). The choice of
gradient is a key cost and performance parameter, since it dictates
the length of the linacs, while the cavity quality factor %{\it }
($Q_0$) relates to the required cryogenic cooling power. The
achievement of 31.5 MV/m as the baseline average operational
accelerating gradient -- requiring a minimum performance of 35 MV/m
during cavity mass-production acceptance testing -- represents the
primary challenge to the global ILC R\&D

With the completion of the RDR, the GDE will begin an
engineering design study, closely coupled with a prioritized R\&D
program. The goal is to produce an Engineering Design Report (EDR) by
2010, presenting the matured technology, design and construction plan
for the ILC, allowing the world High Energy Physics community to seek
government-level project approvals, followed by start of construction
in 2012. When combined with the seven-year construction phase that is
assumed in studies presented in RDR, this timeline will allow
operations to begin in 2019. This is consistent with a technically
driven schedule for this international project.

%\clearpage

\input{resetcounters}

\section{Superconducting RF}

The primary cost driver for the ILC is the superconducting RF
technology used for the Main Linacs, bunch compressors and injector
linacs. In 1992, the TESLA Collaboration began R\&D on 1.3 GHz
technology with a goal of reducing the cost per MeV by a factor of 20
over the then state-of-the-art SCRF installation (CEBAF). This was
achieved by increasing the operating accelerating gradient by a factor
of five from ~5 MV/m to ~25 MV/m, and reducing the cost per meter of
the complete accelerating module by a factor of four for large-scale
production.

\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder tesla9cell.pdf}
  \caption{A TESLA nine-cell 1.3 GHz superconducting niobium cavity.}
  \label{fig:OVtesla9cell}
\end{center}
\end{figure}

The TESLA cavity R\&D was based on extensive existing experience from
CEBAF (Jefferson Lab), CERN, Cornell University, KEK, Saclay and
Wuppertal. The basic element of the technology is a nine-cell 1.3 GHz
niobium cavity, shown in Figure~\ref{fig:OVtesla9cell}. Approximately
160 of these cavities have been fabricated by industry as part of the
on-going R\&D program at DESY; some 17,000 are needed for the ILC.

A single cavity is approximately 1 m long. The cavities must be
operated at 2 K to achieve their performance. Eight or nine cavities are
mounted together in a string and assembled into a common
low-temperature cryostat or {\it cryomodule}
(Figure~\ref{fig:OVcryomodule}), the design of which is already in the
third generation. Ten cryomodules have been produced to-date, five of
which are currently installed in the in the VUV free-electron laser
(FLASH)\footnote{Originally known as the TESLA Test Facility (TTF).}
at DESY, where they are routinely operated. DESY is currently
preparing for the construction of the European XFEL facility, which
will have a $\sim20$ GeV superconducting linac containing 116
cryomodules.


\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder cryomodule.pdf}
  \caption{ SCRF Cryomodules. Left: an 8 cavity TESLA cryomodule is
    installed into the FLASH linac at DESY. Right: design for the 4th
    generation ILC prototype cryomodule, due to be constructed at
    Fermilab National Laboratory.}
  \label{fig:OVcryomodule}
\end{center}
\end{figure}

The ILC community has set an aggressive goal of routinely
achieving\footnote{Acceptance test.} 35 MV/m in nine-cell cavities,
with a minimum production yield of 80\%. Several cavities have already
achieved these and higher gradients (see
Figure~\ref{fig:OV9cellperf}), demonstrating proof of
principle. Records of over 50 MV/m have been achieved in single-cell
cavities at KEK and Cornell\cite{high-g}. However, it is still a challenge
to achieve the desired production yield for nine-cell cavities
at the mass-production levels ($\sim$17,000 cavities) required.

%\begin{comment}
\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder 9cellperf.pdf}
  \caption{High-performance nine-cell cavities. Left: Examples of DESY
    nine-cell cavities achieving $\ge 35$ MV/m. Right: Recent result
    from Jefferson Lab of nine-cell cavity achieving ~40 MV/m.  }
  \label{fig:OV9cellperf}
\end{center}
\end{figure}
%\end{comment}
The key to high-gradient performance is the ultra-clean and
defect-free inner surface of the cavity. Both cavity preparation and
assembly into cavity strings for the cryomodules must be performed in
clean-room environments (Figure~\ref{fig:OVcleanrm}).

\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder cleanrm.pdf}
  \caption{ Clean room environments are mandatory. Left: the assembly
    of eight nine-cell TESLA cavities into a cryomodule string at
    DESY. Right: an ICHIRO nine-cell cavity is prepared for initial
    tests at the Superconducting RF Test Facility (STF) at KEK. }
  \label{fig:OVcleanrm}
\end{center}
\end{figure}

The best
cavities have been achieved using electropolishing, a common industry
practice which was first developed for use with superconducting
cavities by CERN and KEK. Over the last few years, research at
Cornell, DESY, KEK and Jefferson Lab has led to an agreed standard
procedure for cavity preparation, depicted in
Figure~\ref{fig:OVcavproc}. The focus of the R\&D is now to optimize
the process to guarantee the required yield. The ILC SCRF community
has developed an internationally agreed-upon plan to address the
priority issues.


\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder cavproc.pdf}
  \caption{ Birth of a nine-cell cavity: basic steps in surface
    treatment needed to achieve high-performance superconducting
    cavities. (EP = electropolishing; HPR = high-pressure rinsing.) }
  \label{fig:OVcavproc}
\end{center}
\end{figure}

The high-gradient SCRF R\&D required for ILC is expected to ramp-up
world-wide over the next years. The U.S. is currently investing in new
infrastructure for nine-cell cavity preparation and string and
cryomodule assembly. These efforts are centered at Fermilab (ILC Test
Accelerator, or ILCTA), together with ANL, Cornell University, SLAC
and Jefferson Lab. In Japan, KEK is developing the
Superconducting RF Test Facility (STF). In Europe, the focus of R\&D at
DESY has shifted to industrial preparation for construction of the
XFEL. There is continued R\&D to support the high-gradient program, as
well as other critical ILC-related R\&D such as high-power RF couplers
(LAL, Orsay, France) and cavity tuners (CEA Saclay, France; INFN
Milan, Italy).

The quest for high-gradient and affordable SCRF technology for
high-energy physics has revolutionized accelerator applications. In addition
to the recently completed Spallation Neutron Source (SNS) in Oak Ridge, Tennessee and the European XFEL under construction, many linac-based
projects utilizing
SCRF technology are being developed, including 4th-generation light
sources such as single-pass FELs and energy-recovery linacs. For the large
majority of new accelerator-based projects, SCRF has become the
technology of choice.

%\clearpage

\input{resetcounters}
\section{The ILC Baseline Design}\label{Ovr:baseline}

The overall system design has been chosen to realize the physics
requirements with a maximum CM energy of 500 GeV and a peak luminosity
of $2\times10^{34}$ cm$^{-2}$s$^{-1}$. Figure~\ref{fig:OVlayout} shows
a schematic view of the overall layout of the ILC, indicating the
location of the major sub-systems:

\begin{itemize}

  \item a polarized electron source based on a photocathode DC gun;
  \item an undulator-based positron source, driven by a the 150 GeV
    main electron beam;
  \item 5 GeV electron and positron damping rings (DR) with a
    circumference of 6.7 km, housed in a common tunnel at the center
    of the ILC complex;
  \item beam transport from the damping rings to the main linacs,
    followed by a two-stage bunch compressor system prior to injection into the
    main linac;
  \item two 11 km long main linacs, utilizing 1.3 GHz SCRF cavities,
    operating at an average gradient of 31.5 MV/m, with a pulse length
    of 1.6 ms;
  \item a 4.5 km long beam delivery system, which brings the two beams
    into collision with a 14 mrad crossing angle, at a single
    interaction point which can be shared by two detectors.

\end{itemize}

\begin{figure}[htb]
\begin{center}
  \includegraphics[width=8.5cm]{\picturefolder layout.pdf}
  \caption{Schematic layout of the ILC complex for 500 GeV CM.}
  \label{fig:OVlayout}
\end{center}
\end{figure}

The total footprint is $\sim$31 km. The electron source, the damping
rings, and the positron auxiliary (`keep-alive') source are centrally
located around the interaction region (IR). The plane of the damping
rings is elevated by $\sim$10 m above that of the BDS to avoid
interference.

To upgrade the machine to $E_{\rm cms} =1$ TeV, the linacs and the beam
transport lines from the damping rings would be extended by another
$\sim 11$ km each. Certain components in the beam delivery system
would also need to be augmented or replaced.

\subsection{Beam Parameters}

\begin{table}[htb]
\caption{ Basic design parameters for the ILC. $^{a)}$at 500GeV
  center-of-mass energy. \label{tab:BaseParams}}
\begin{center}
    \begin{tabular}{lll}\\ \hline
    Parameter                   & Unit              &          \\ \hline
    Center-of-mass energy range & GeV               & 200 - 500         \\
    Peak luminosity$^{a)}$      & cm$^{-2}$s$^{-1}$ & $2\times 10^{34}$ \\
                                &                   &                   \\
    Beam current                & mA                & 9.0               \\
    Pulse rate                  & Hz                & 5.0               \\
    Pulse length (beam)         & ms                & $\sim1$           \\
    Number of bunches per pulse &                   & 1000 - 5400       \\
    Charge per bunch            & nC                & 1.6 - 3.2         \\
    Accelerating gradient$^{a)}$      & MV/m        & 31.5              \\
    RF pulse length             & ms                & 1.6               \\
    Beam power (per beam)$^{a)}$      & MW          & 10.8              \\
                                &                   &                   \\
    Typical beam size at IP$^{a)}$ ($h\times v$) & nm & 640 $\times$ 5.7\\
                                &                   &                   \\
    Total AC Power consumption$^{a)}$ &MW           & 230               \\
    \hline
    \end{tabular}
\end{center}
\end{table}

The nominal beam parameter set, corresponding to the design luminosity
of $2\times10^{34}$ cm$^{-2}$s$^{-1}$ at $E_{\rm cms} = 500$ GeV is given in Table~\ref{tab:BaseParams}. These parameters have been chosen to optimize between known accelerator physics and technology
challenges throughout the whole accelerator complex. Examples of such
challenges are:

\begin{itemize}

  \item beam instability and kicker hardware constraints in the
    damping rings;

  \item beam current, beam power, and pulse length limitations in the
    main linacs;

  \item emittance preservation requirements, in the main linacs and
    the beam delivery system;

  \item background control and kink instability issues in the interaction region.

\end{itemize}

Nearly all high-energy physics accelerators have shown unanticipated
difficulties in reaching their design luminosity. The ILC design
specifies that each subsystem support a range of beam parameters. The
resulting flexibility in operating parameters will allow identified
problems in one area to be compensated for in another. The nominal IP
beam parameters and design ranges are presented in
Table~\ref{tab:OVparamrange}.


\begin{table}[htb]
\begin{center}
\begin{tabular}{lrrrl} \hline
             &  min  & nominal. & max. & unit \\ \hline
Bunch population                            & 1       & 2      & 2    & $\times10^{10}$ \\
Number of bunches                           & 1260    & 2670   & 5340 &                 \\
Linac bunch interval                        & 180     & 369    & 500  & ns              \\
RMS bunch length                            & 200     & 300    & 500  & $\mu$m          \\
Normalized horizontal emittance at IP       & 10      & 10     & 12   & mm$\cdot$mrad   \\
Normalized vertical emittance at IP         & 0.02    & 0.04   & 0.08 & mm$\cdot$mrad   \\
Horizontal beta function at IP              & 10      & 20     & 20   & mm              \\
Vertical beta function at IP                & 0.2     & 0.4    & 0.6  & mm              \\
RMS horizontal beam size at IP              & 474     & 640    & 640  & nm              \\
RMS vertical beam size at IP                & 3.5     & 5.7    & 9.9  & nm              \\
Vertical disruption parameter               & 14      & 19.4   & 26.1 &                 \\
Fractional RMS energy loss to beamstrahlung &   1.7   &  2.4  &   5.5 &  \% \\
\hline
\end{tabular}
\caption{Nominal and design range of beam parameters at the IP. The
  min. and max. columns do not represent consistent sets of
  parameters, but only indicate the span of the design range for each
  parameter. (Nominal vertical emittance assumes a 100\% emittance
  dilution budget from the damping ring to the IP.)}
\label{tab:OVparamrange}
\end{center}
\end{table}

\subsection{Electron Source}

\subparagraph{Functional Requirements} \\

The ILC polarized electron source must:
\begin{itemize}
  \item generate the required bunch train of polarized electrons
       ($>80\%$ polarization);
  \item capture and accelerate the beam to 5 GeV;
  \item transport the beam to the electron damping ring with minimal
       beam loss, and perform an energy compression and spin rotation
       prior to injection.
\end{itemize}

\subparagraph{System Description} \\

The polarized electron source is located on the positron linac side of
the damping rings. The beam is produced by a laser illuminating a
photocathode in a DC gun. Two independent laser and gun systems
provide redundancy. Normal-conducting structures are used for bunching
and pre-acceleration to 76 MeV, after which the beam is accelerated to
5 GeV in a superconducting linac. Before injection into the damping
ring, superconducting solenoids rotate the spin vector into the
vertical, and a separate superconducting RF structure is used for
energy compression. The layout of the polarized electron source is
shown in Figure~\ref{fig:OVPES}.


\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder PES.pdf}
  \caption{Schematic View of the Polarized Electron Source.}
  \label{fig:OVPES}
\end{center}
\end{figure}

\subparagraph{Challenges} \\

The SLC polarized electron source already meets the requirements for
polarization, charge and lifetime. The primary challenge for the ILC
electron source is the ~1 ms long bunch train, which demands a laser
system beyond that used at any existing accelerator.

\subsection{Positron Source}

\subparagraph{Functional requirements} \\
The positron source must perform several critical functions:

\begin{itemize}

  \item generate a high-power multi-MeV photon production drive beam
    in a suitably short-period, high K-value helical undulator;

  \item produce the needed positron bunches in a metal target that can
    reliably deal with the beam power and induced radioactivity;

  \item capture and accelerate the beam to 5 GeV;

  \item transport the beam to the positron damping ring with minimal
    beam loss, and perform an energy compression and spin rotation
    prior to injection.
\end{itemize}

\subparagraph{System Description} \\

The major elements of the ILC positron source are shown in
Figure~\ref{fig:OVposi}. The source uses photoproduction to generate
positrons. After acceleration to 150 GeV, the electron beam is
diverted into an offset beamline, transported through a 150-meter
helical undulator, and returned to the electron linac. The high-energy
($\sim$10 MeV) photons from the undulator are directed onto a rotating
0.4 radiation-length Ti-alloy target $\sim$500 meters downstream,
producing a beam of electron and positron pairs. This beam is then
matched using an optical-matching device into a normal conducting (NC)
L-band RF and solenoidal-focusing capture system and accelerated to
125 MeV. The electrons and remaining photons are separated from the
positrons and dumped. The positrons are accelerated to 400 MeV in a NC
L-band linac with solenoidal focusing. The beam is transported ~5 km
through the rest of the electron main linac tunnel, brought to the
central injector complex, and accelerated to 5 GeV using
superconducting L-band RF. Before injection into the damping ring,
superconducting solenoids rotate the spin vector into the vertical,
and a separate superconducting RF structure is used for energy
compression.

The baseline design is for unpolarized positrons, although the beam
has a polarization of 30\%, and beamline space has been reserved for
an eventual upgrade to 60\% polarization.

To allow commissioning and tuning of the positron systems while the
high-energy electron beam is not available, a low-intensity auxiliary
(or ``keep-alive'') positron source is provided. This is a
conventional positron source, which uses a 500 MeV electron beam
impinging on a heavy-metal target to produce $\sim$10\% of the nominal
positron beam.  The keep-alive and primary sources use the same linac
to accelerate from 400 MeV to 5 GeV.


\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder posi.pdf}
  \caption{Overall Layout of the Positron Source.}
  \label{fig:OVposi}
\end{center}
\end{figure}

\subparagraph{Challenges} \\

The most challenging elements of the positron source are:

\begin{itemize}

  \item the 150 m long superconducting helical undulator, which has a
    period of 1.15 cm and a K-value of 0.92, and a 6 mm inner diameter
    vacuum chamber;

  \item the Ti-alloy target, which is a cylindrical wheel 1.4 cm thick
    and 1 m in diameter, which must rotate at 100 m/s in vacuum to
    limit damage by the photon beam;

  \item the normal-conducting RF system which captures the positron
    beam, which must sustain high accelerator gradients during
    millisecond-long pulses in a strong magnetic field, while
    providing adequate cooling in spite of high RF and particle-loss
    heating.

\end{itemize}

The target and capture sections are also high-radiation areas which
present remote handing challenges.

\subsection{Damping Rings}

\subparagraph{Functional requirements} \\
The damping rings must perform four critical functions:

\begin{itemize}

  \item accept $e^-$ and $e^+$ beams with large transverse and
    longitudinal emittances and damp to the low emittance beam
    required for luminosity production (by five orders of magnitude
    for the positron vertical emittance), within the 200 ms between
    machine pulses;

  \item inject and extract individual bunches without affecting the
    emittance or stability of the remaining stored bunches;

  \item damp incoming beam jitter (transverse and longitudinal) and
    provide highly stable beams for downstream systems;

  \item delay bunches from the source to allow feed-forward systems to
    compensate for pulse-to-pulse variations in parameters such as the
    bunch charge.

\end{itemize}

\subparagraph{System Description} \\

The ILC damping rings include one electron and one positron ring, each
6.7 km long, operating at a beam energy of 5 GeV. The two rings are
housed in a single tunnel near the center of the site, with one ring
positioned directly above the other. The plane of the DR tunnel is
located $\sim$10 m higher than that of the beam delivery system.  This
elevation difference gives adequate shielding to allow operation of
the injector system while other systems are open to human access.

The damping ring lattice is divided into six arcs and six straight
sections. The arcs are composed of TME cells; the straight sections
use a FODO lattice. Four of the straight sections contain the RF
systems and the superconducting wigglers. The remaining two sections
are used for beam injection and extraction. Except for the wigglers,
all of the magnets in the ring, are normal-conducting. Approximately
200 m of superferric wigglers are used in each damping ring. The
wigglers are 2.5 m long devices, operating at 4.5K, with a peak field
of 1.67 T.

The superconducting RF system is operated CW at 650 MHz, and provides
24 MV for each ring. The frequency is chosen to be half the linac RF frequency to easily accommodate different bunch patterns.  The single-cell cavities
operate at 4.5 K and are housed in eighteen 3.5 m long
cryomodules. Although a number of 500 MHz CW RF systems are currently
in operation, development work is required for this 650 MHz system,
both for cavities and power sources.

The momentum compaction of the lattice is relatively large, which
helps to maintain single bunch stability, but requires a relatively
high RF voltage to achieve the design RMS bunch length (9 mm). The
dynamic aperture of the lattice is sufficient to allow the large
emittance injected beam to be captured with minimal loss.


\subparagraph{Challenges} \\

The principal challenges in the damping ring are:
\begin{itemize}

  \item control of the electron cloud effect in the positron damping
    ring. This effect, which can cause instability, tune spread, and
    emittance growth, has been seen in a number of other rings and is
    relatively well understood. Simulations indicate that it can be
    controlled by proper surface treatment of the vacuum chamber to
    suppress secondary emission, and by the use of solenoids and
    clearing electrodes to suppress the buildup of the cloud.

  \item control of the fast ion instability in the electron damping
    ring. This effect can be controlled by limiting the pressure in
    the electron damping ring to below 1 nTorr, and by the use of
    short gaps in the ring fill pattern.

  \item development of a very fast rise and fall time kicker for single
    bunch injection and extraction in the ring. For the most demanding
    region of the beam parameter range, the bunch spacing in the
    damping ring is $\sim$3 ns, and the kicker must have a rise plus fall
    time no more than twice this. Short stripline kicker structures
    can achieve this, but the drive pulser technology still needs
    development.

\end{itemize}

\subsection{Ring to Main Linac (RTML)}
\subparagraph{Functional requirements} \\
The RTML must perform several critical functions for each beam:

\begin{itemize}

  \item transport the beam from the damping ring to the upstream end
    of the linac;

  \item collimate the beam halo generated in the damping ring;

  \item rotate the polarization from the vertical to any arbitrary
    angle required at the IP;

  \item compress the long Damping Ring bunch length by a factor of
    $30\sim45$ to provide the short bunches required by the Main Linac
    and the IP;

\end{itemize}

\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder RTML.pdf}
  \caption{Schematic of the RTML.}
  \label{fig:OVRTML}
\end{center}
\end{figure}

\subparagraph{System Description} \\

The layout of the RTML is identical for both electrons and positrons,
and is shown in Figure~\ref{fig:OVRTML}. The RTML consists of the
following subsystems:

\begin{itemize}
  \item an $\sim$15 km long 5 GeV transport line;

  \item betatron and energy collimation systems;

  \item a $180^{\circ}$ turn-around, which enables feed-forward beam
    stabilization;

  \item spin rotators to orient the beam polarization to the desired
    direction;

  \item a 2-stage bunch compressor to compress the beam bunch length
    from several millimeters to a few hundred microns as required at
    the IP.

\end{itemize}

The bunch compressor includes acceleration from 5 GeV to 13-15 GeV in
order to limit the increase in fractional energy spread associated
with bunch compression.

\subparagraph{Challenges} \\

The principal challenges in the RTML are:
\begin{itemize}

  \item control of emittance growth due to static misalignments,
    resulting in dispersion and coupling. Simulations indicate that
    the baseline design for beam-based alignment can limit the
    emittance growth to tolerable levels.

  \item suppression of phase and amplitude jitter in the bunch
    compressor RF, which can lead to timing errors at the IP. RMS
    phase jitter of 0.24$^{\circ}$ between the electron and positron
    RF systems results in a 2\% loss of luminosity. Feedback loops in
    the bunch compressor low-level RF system should be able to limit
    the phase jitter to this level.
\end{itemize}

&\clearpage

\input{resetcounters}
\section{Main Linacs}

\subparagraph{Functional requirements} \\

The two main linacs accelerate the electron and positron beams from
their injected energy of 15 GeV to the final beam energy of 250 GeV,
over a combined length of 23 km. The main linacs must:

\begin{itemize}

  \item accelerate the beam while preserving the small bunch
    emittances, which requires precise orbit control based on data
    from high resolution beam position monitors, and also requires
    control of higher-order modes in the accelerating cavities;

  \item maintain the beam energy spread within the design requirement
    of $\sim$0.1~\% at the IP;

  \item not introduce significant transverse or longitudinal jitter,
    which could cause the beams to miss at the collision point.

\end{itemize}

\subparagraph{System description} \\

The ILC Main Linacs accelerate the beam from 15 GeV to a maximum
energy of 250 GeV at an average accelerating gradient of 31.5
MV/m. The linacs are composed of RF units, each of which are formed by
three contiguous SCRF cryomodules containing 26 nine-cell
cavities. The layout of one unit is illustrated in
Figure~\ref{fig:OVRFunit}. The positron linac contains 278 RF units,
and the electron linac has 282 RF units\footnote{Approximate 3 GeV of
  extra energy is required in the electron linac to compensate for
  positron production.}.

\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder RFunit.pdf}
  \caption{RF unit layout.}
  \label{fig:OVRFunit}
\end{center}
\end{figure}

Each RF unit has a stand-alone RF source, which includes a
conventional pulse-transformer type high-voltage (120 kV) modulator, a
10 MW multi-beam klystron, and a waveguide system that distributes the
RF power to the cavities (see Figure~\ref{fig:OVRFunit}). It also
includes the low-level RF (LLRF) system to regulate the cavity field
levels, interlock systems to protect the source components, and the
power supplies and support electronics associated with the operation
of the source.

The cryomodule design is a modification of the Type-3 version
(Figure~\ref{fig:OVcryomodule}) developed and used at DESY. Within the
cryomodules, a 300 mm diameter helium gas return pipe serves as a
strongback to support the cavities and other beam line components.
The middle cryomodule in each RF unit contains a quad package that
includes a superconducting quadrupole magnet at the center, a cavity
BPM, and superconducting horizontal and vertical corrector
magnets. The quadrupoles establish the main linac magnetic lattice,
which is a weak focusing FODO optics with an average beta function of
$\sim$80 m. All cryomodules are 12.652 m long, so the active-length to
actual-length ratio in a nine-cavity cryomodule is 73.8\%. Every
cryomodule also contains a 300 mm long high-order mode beam absorber
assembly that removes energy through the 40-80 K cooling system from
beam-induced higher-order modes above the cavity cutoff frequency.


To operate the cavities at 2 K, they are immersed in a saturated He II
bath, and helium gas-cooled shields intercept thermal radiation and
thermal conduction at 5-8 K and at 40-80 K. The estimated static and
dynamic cryogenic heat loads per RF unit at 2 K are 5.1 W and 29 W,
respectively. Liquid helium for the main linacs and the RTML is
supplied from 10 large cryogenic plants, each of which has an
installed equivalent cooling power of $\sim$20 kW at 4.5 K. The main
linacs follow the average Earth's curvature to simplify the liquid
helium transport.

The Main Linac components are housed in two tunnels, an accelerator
tunnel and a service tunnel, each of which has an interior diameter of
4.5 meters. To facilitate maintenance and limit radiation exposure,
the RF source is housed mainly in the service tunnel as illustrated in
Figure~\ref{fig:OVtunnel}.

\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder tunnel.pdf}
  \caption{Cutaway view of the linac dual-tunnel configuration.}
  \label{fig:OVtunnel}
\end{center}
\end{figure}

The tunnels are typically hundreds of meters underground and are
connected to the surface through vertical shafts\footnote{Except for
  the Asian sample site: see section 1.4.}. Each of the main linacs
includes three shafts, roughly 5 km apart as dictated by the cryogenic
system. The upstream shafts in each linac have diameters of 14 m to
accommodate lowering cryomodules horizontally, and the downstream
shaft in each linac is 9 m in diameter, which is the minimum size
required to accommodate tunnel boring machines. At the base of each
shaft is a 14,100 cubic meter cavern for staging installation; it also houses[BF1] utilities and parts of the cryoplant, most of which are
located on the surface.

\subparagraph{Challenges} \\
The principal challenges in the main linac are:
\begin{itemize}

  \item achieving the design average accelerating gradient of 31.5
    MV/m. This operating gradient is higher than that typically
    achievable today and assumes further progress will be made during
    the next few years in the aggressive program that is being pursued
    to improve cavity performance.

  \item control of emittance growth due to static misalignments,
    resulting in dispersion and coupling. Beam-based alignment
    techniques should be able to limit the single-bunch emittance
    growth. Long-range multibunch effects are mitigated via HOM
    damping ports on the cavities, HOM absorbers at the quadrupoles,
    and HOM detuning. Coupling from mode-rotation HOMs is limited by
    splitting the horizontal and vertical betatron tunes.

  \item control of the beam energy spread. The LLRF system monitors
    the vector sum of the fields in the 26 cavities of each RF unit
    and makes adjustments to flatten the energy gain along the bunch
    train and maintain the beam-to-RF phase constant. Experience from
    FLASH and simulations indicate that the baseline system should
    perform to specifications.

\end{itemize}

%-----------------------------------------------------

\subsection{Beam Delivery System}

\subparagraph{Functional requirements} \\

The ILC Beam Delivery System (BDS) is responsible for transporting the
$e^+e^-$ beams from the exit of the high energy linacs, focusing them to
the sizes required to meet the ILC luminosity goals, bringing them
into collision, and then transporting the spent beams to the main beam
dumps. In addition, the BDS must perform several other critical
functions:

\begin{itemize}

  \item measure the linac beam and match it into the final focus;

  \item protect the beamline and detector against mis-steered beams
    from the main linacs;

  \item remove any large amplitude particles (beam-halo) from the
    linac to minimize background in the detectors;

  \item measure and monitor the key physics parameters such as energy
    and polarization before and after the collisions.

\end{itemize}

\subparagraph{System Description} \\

The layout of the beam delivery system is shown in
Figure~\ref{fig:OVBDS}. There is a single collision point with a 14
mrad total crossing angle. The 14 mrad geometry provides space for
separate extraction lines but requires crab cavities to rotate the
bunches in the horizontal plane for effective head-on
collisions. There are two detectors in a common interaction region
(IR) hall in a so-called ``push-pull'' configuration. The detectors
are pre-assembled on the surface and then lowered into the IR hall
when the hall is ready for occupancy.

The BDS is designed for 500 GeV center-of-mass energy but can be
upgraded to 1 TeV with additional magnets.


\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder BDS.pdf}
  \caption{BDS layout, beam and service tunnels (shown in magenta and
    green), shafts, experimental hall.  The line crossing the BDS
    beamline at right angles is the damping ring, located 10 m above
    the BDS tunnels.}
  \label{fig:OVBDS}
\end{center}
\end{figure}

The BDS is designed for 500 GeV center-of-mass energy but can be
upgraded to 1 TeV with additional magnets.

The main subsystems of the beam delivery, starting from the exit of
the main linacs, are:

\begin{itemize}

  \item a section containing post-linac emittance measurement and
    matching (correction) sections, trajectory feedback, polarimetry
    and energy diagnostics;

  \item a fast pulsed extraction system used to extract beams in case
    of a fault, or to dump the beam when not needed at the IP;

  \item a collimation section which removes beam halo particles that
    would otherwise generate unacceptable background in the detector,
    and also contains magnetized iron shielding to deflect muons;

  \item the final focus (FF) which uses strong compact superconducting
    quadrupoles to focus the beam at the IP, with sextupoles providing
    local chromaticity correction;

  \item the interaction region, containing the experimental
    detectors. The final focus quadrupoles closest to the IP are
    integrated into the detector to facilitate detector ``push-pull'';

   \item the extraction line, which has a large enough bandwidth to
     cleanly transport the heavily disrupted beam to a high-powered
     water-cooled dump. The extraction line also contains important
     polarization and energy diagnostics.

\end{itemize}

\subparagraph{Challenges} \\
The principal challenges in the beam delivery system are:
\begin{itemize}
  \item tight tolerances on magnet motion (down to tens of
    nanometers), which make the use of fast beam-based feedback
    systems mandatory, and may well require mechanical stabilization
    of critical components (e.g. final doublets).

  \item uncorrelated relative phase jitter between the crab cavity
    systems, which must be limited to the level of tens of
    femtoseconds.

  \item control of emittance growth due to static misalignments, which
    requires beam-based alignment and tuning techniques similar to the
    RTML.

  \item control of backgrounds at the IP via careful tuning and
    optimization of the collimation systems and the use of the
    tail-folding octupoles.

  \item clean extraction of the high-powered disrupted beam to the
    dump. Simulations indicate that the current design is adequate
    over the full range of beam parameters.
\end{itemize}


%\clearpage

\input{resetcounters}
\section{Sample Sites}


Conventional Facilities and Siting (CFS) is responsible for civil
engineering, power distribution, water cooling and air conditioning
systems. The value estimate (see Section~\ref{sec:ValueEstimate})
for the CFS is approximately 38\% of the total estimated
project value.

In the absence of a single agreed-upon location for the ILC, a sample
site in each region was developed. Each site was designed to support
the baseline design described in Section~\ref{Ovr:baseline}. Although many of the basic requirements are identical, differences in geology, topography
and local standards and regulations lead to different construction
approaches, resulting in a slight variance in value estimates across
the three regions. Although many aspects of the CFS (and indeed
machine design) will ultimately depend on the specific host site
chosen, the approach taken here is considered sufficient for the
current design phase, while giving a good indication of the influence
of site-specific issues on the project as a whole.

Early in the RDR process, the regional CFS groups agreed upon a matrix of criteria for any sample site. All three sites satisfied these criteria, including the mandatory requirement that the site can support the extension to the 1 TeV
center-of-mass machine.



\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder sitesec.pdf}
  \caption{Geology and tunnel profiles for the three regional sites,
    showing the location of the major access shafts (tunnels for the
    Asian site). Top: the Americas site close to Fermilab. Middle: the
    Asian site in Japan. Bottom: the European site close to CERN.}
  \label{fig:OVsitesec}
\end{center}
\end{figure}

The three sample sites have the following characteristics:

\begin{itemize}

  \item The Americas sample site lies in Northern Illinois near Fermilab.
    The site provides a range of locations to
    position the ILC in a north-south orientation. The site chosen has
    approximately one-quarter of the machine on the Fermilab site. The
    surface is primarily flat. The long tunnels are bored in a
    contiguous dolomite rock strata (¡ÆGalena Platteville¡Ç), at a
    typical depth of 30-100 m below the surface.

  \item The Asian site has been chosen from several possible ILC
    candidate sites in Japan. The sample site has a uniform terrain
    located along a mountain range, with a tunnel depth ranging from
    40 m to 600 m. The chosen geology is uniform granite highly suited
    to modern tunneling methods. One specific difference for the Asian
    site is the use of long sloping access tunnels instead of vertical
    shafts, the exception being the experimental hall at the
    Interaction Region, which is accessed via two 112 m deep vertical
    shafts. The sloping access tunnels take advantage of the
    mountainous location.

  \item The European site is located at CERN, Geneva, Switzerland, and
    runs parallel to the Jura mountain range, close to the CERN
    site. The majority of the machine is located in the `Molasse' (a
    local impermeable sedimentary rock), at a typical depth of 370 m.

\end{itemize}

The elevations of the three sample sites are shown in
Figure~\ref{fig:OVsitesec}. The tunnels for all three sites would be
predominantly constructed using Tunnel Boring Machines (TBM), at
typical rates of 20--30 m per day. The Molasse of the European site
near CERN requires a reinforced concrete lining for the entire tunnel
length. The Asian site (granite) requires rock bolts and a 5 cm
`shotcrete' lining. The US site is expected to require a concrete
lining for only approximately 20\% of its length, with rock-bolts
being sufficient for permanent structural support.

A second European sample site near DESY, Hamburg, Germany, has also
been developed. This site is significantly different from the three
reported sites, both in geology and depth (~25 m deep), and requires
further study.

In addition, the Joint Institute for Nuclear Research has submitted a
proposal to site the ILC in the neighborhood of Dubna, Russian
Federation.

The three sites reported in detail here are all `deep-tunnel'
solutions. The DESY and Dubna sites are examples of `shallow' sites. A
more complete study of shallow sites -- shallow tunnel or
cut-and-cover -- will be made in the future as part of the Engineering
Design phase.


\clearpage
\input{resetcounters}
\chapter{Detectors}
\input{Detectors}

\clearpage
\input{resetcounters}
\chapter{Value Estimates}\label{sec:ValueEstimate}
\section{The Accelerator}

A preliminary cost analysis has been performed for the ILC Reference
Design.  A primary goal of the estimate was to allow
cost-to-performance optimization in the Reference Design, before
entering into the engineering design phase.  Over the past year, the
component costs were estimated, various options compared and the
design evolved through about ten significant cost-driven changes,
resulting in a cost reduction of about 25\%, while still maintaining
the physics performance goals.

The ILC cost estimates have been performed using a ``value'' costing
system, which provides basic agreed-to value costs for components in
ILC Units\footnote{For this value estimate, 1 ILC Unit = 1 US 2007\$
  (= 0.83 Euro = 117 Yen).}, and an estimate of the explicit labor (in
person hours) that is required to support the project.  The estimates
are based on making world-wide tenders (major industrialized nations),
using the lowest reasonable price for the required quality.  There are
three classes of costs:

\begin{itemize}
  \item site-specific costs, where a separate estimate was made in
    each of the three regions;
  \item conventional costs for items where there is global capability
    -- here a single cost was determined;
  \item costs for specialized high-tech components (e.g. the SCRF linac
    technology), where industrial studies and engineering estimates
    were used.
\end{itemize}

The total estimated value for the shared ILC costs for the Reference
Design is 4.79 Billion (ILC Units). An important outcome of the value
costing has been to provide a sound basis for determining the relative
value of the various components or work packages. This will enable
equitable division of the commitments of the world-wide collaboration.

In addition, the site specific costs, which are related to the direct
costs to provide the infrastructure required to site the machine, are
estimated to be 1.83 Billion (ILC Units). These costs include the
underground civil facilities, water and electricity distribution and
buildings directly supporting ILC operations and construction on the
surface.  The costs were determined to be almost identical for the
Americas, Asian, and European sample sites. It should be noted that
the actual site-specific costs will depend on where the machine is
constructed, and the facilities that already exist at that location.

Finally, the explicit labor required to support the construction
project is estimated at 24 million person-hours; this includes
administration and project management, installation and testing.  This
labor may be provided in different ways, with some being contracted
and some coming from existing labor in collaborating institutions.

The ILC Reference Design cost estimates and the tools that have been
developed will play a crucial role in the engineering design effort,
both in terms of studying options for reducing costs or improving
performance, and in guiding value engineering studies, as well as
supporting the continued development of a prioritized R\&D program.

The total estimated value cost for the ILC, defined by the Reference
Design, including shared value costs, site specific costs and explicit
labor, is comparable to other recent major international projects,
e.g. ITER, and the CERN LHC when the cost of pre-existing facilities
are taken into account. The GDE is confident that the overall scale of
the project has been reliably estimated and that cost growth can be
contained in the engineering phase, leading to a final project cost
consistent with that determined at this early stage in the design.

\section{The Detectors}

Three detector concepts, GLD, LDC, and SiD, estimated the costs of their respective detector designs. Each used a complete work breakdown structure, and identified the significant costs associated with subsystems, and costs associated with assembly and installation. Estimates were guided by the GDE costing rules. The three estimates are reasonably consistent to 20\%, but are divided differently between M\&S and labor, a result of regional accounting differences.

The cost drivers for the M\&S budgets are the calorimeters and the solenoidal magnet and flux return iron. Integration, transportation, and computing have been included, as have indirect costs associated with both M&S and labor.

The coil costs for each of the concepts were consistent with the costs for the BaBar, Aleph, and CMS coils when compared as a function of stored energy. The cost breakdowns across detector subsystems for each of three concepts differ concept to concept.  This is to be expected, as SiD has costed electronics, installation, and management as separate items whereas LDC and GLD have embedded these in the subdetectors. In another example, GLD chooses to cost both hadron and electromagnetic calorimeters as a single item, since the detectors used are similar. LDC and SiD have separated these expenses, because the detection techniques are quite different.

Based on the SiD and LDC estimates, the value (M\&S) cost is in the range 260-360 Million (ILC Units).  GLD does not estimate M\&S separately.  Manpower for SiD and LDC is estimated at 1000-1300 person-years.  Combining M\&S and person-years, the total detector cost lies in the range of 400-500 Million (ILC Units) for any of the detector concepts. The cost scale for the two detectors envisioned for the ILC is about 10\% of the cost of the machine.


\clearpage

\input{resetcounters}
\chapter{Next Steps: R\&D and the Engineering Design Phase}
\section{Accelerator R\&D}

For the last year, the focus of the core GDE activity has been on
producing the RDR and value estimate. In parallel, ILC R\&D programs
around the world have been ramping up to face the considerable
challenges ahead. The GDE Global R\&D Board -- a group of twelve GDE
members from the three regions -- has evaluated existing programs, and
has convened task forces of relevant experts to produce an
internationally agreed-upon prioritized R\&D plan for the critical
items. The highest-priority task force (S0/S1) addresses the SCRF
accelerating gradient:

\begin{itemize}
  \item S0: high-gradient cavity -- aiming to achieve 35 MV/m
    nine-cell cavity performance with an 80\% production yield;
  \item S1: high-gradient cryomodule ? the development of one or more
    high-gradient ILC cryomodules with an average operational gradient
    of 31.5 MV/m.

\end{itemize}

The S0/S1 task force has already produced focused and comprehensive
R\&D plans. Other task forces (S2: test linac; S3: Damping Ring; S4:
Beam Delivery System, etc.) are in the process of either completing
their reports, or just beginning their work.

For the cost- and performance-critical SCRF, the primary focus of
S0/S1 remains the baseline choice, the relatively mature TESLA
nine-cell elliptical cavity. However, additional research into
alternative cavity shapes and materials continues in parallel. One
promising technique is the use of `large-grain'
niobium~\cite{large-grain}, as opposed to the small-grain material
that has been used in the past (Figure~\ref{fig:OVcavRD}).  Use of
large grain material may remove the need for electropolishing, since
the same surface finish can potentially be achieved with Buffered
Chemical Polishing (BCP) -- a possible cost saving. Several
single-cells have achieved gradients in excess of 35 MV/m (without
electropolishing) and more recent nine-cell cavity tests have shown
very promising results.

\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.95\textwidth]{\picturefolder cavRD.pdf}
  \caption{Cutting-edge SCRF R\&D. Top-left: ICHIRO single-cells being
    prepared for testing at KEK. Top-right: world-record performance
    from novel shape single-cells (ICHIRO and Cornell's reentrant
    cavity). Bottom-left: large-grain niobium disk (Jefferson
    Lab). Bottom-right: single-cell cavity produced from large-grain
    niobium material (Jefferson Lab).}
  \label{fig:OVcavRD}
\end{center}
\end{figure}

Various new and promising cavity shapes are also being investigated,
primarily at KEK and Cornell. While the basic nine-cell form remains,
the exact shape of the `cells' is modified to reduce the peak magnetic
field at the niobium surface. In principle these new shapes can
achieve higher gradients, or higher quality factors
($Q_0$). Single-cells at KEK (ICHIRO) and Cornell (reentrant) have
achieved the highest gradients to date ($\sim$50 MV/m, see
Figure~\ref{fig:OVcavRD}). R\&D towards making high-performance
nine-cell cavities using these designs continues as future possible
alternatives to the ILC baseline cavity.

The GDE formally supports R&D on alternative designs for components other than the cavities, where the new designs promise potential cost and/or performance benefits. Some key examples are alternative RF power
source components, of which the Marx modulator is currently the most
promising.  In addition, R\&D on critical technologies will
continue through the EDR. Topics include items such as the damping
ring kickers and electron-cloud mitigation techniques, the positron
target and undulator, the magnets around the beam interaction point,
and global issues that require very high availability such as the
control system, the low-level RF, and the magnet power supplies.

\section{Future Detector R\&D}

The detector R\&D and integrated design effort must keep pace with progress on the ILC. The detector R\&D program, which has already developed over many years, includes efforts in all regions, with inter-regional collaboration in some cases, and inter-regional coordination in all cases. The R\&D is reviewed within the global context by the World Wide Study. This R\&D is critical to the success of the ILC experimental program.

To focus effort over the next few years, the current studies for four distinct concepts should be concentrated into no more than two engineering design efforts, ready to be proposed at the same time as the ILC EDR. The two complementary detectors should each have broad international participation. The ILCSC is developing a process to assist this evolution. The two detector designs should be chosen by late 2008 to early 2009, and their engineering designs will then be completed over the next two or three years.

\section{Towards the Engineering Design Report (EDR)}

While investment into the critical R\&D remains a priority, a
significant ramping-up of global engineering resources will now be
required to produce an engineered technical design by 2010. An
important aspect of this work will be the refinement and control of
the published cost estimate by value engineering. The EDR phase will
also require a restructuring of the GDE to support the expanded
scope. A more traditional project structure will be adopted based on
the definition of a discrete set of Work Packages. The responsibility
for achieving the milestones and deliverables of each Work Package
will be assigned to either a single institute, or consortium of
institutes, under the overall coordination of a central project
management team. The Work Packages need to be carefully constructed to
accommodate the direct needs of the Engineering Design phase,
while at the same time reflecting the global nature of the project. An
important goal of the current planning is to integrate the engineering
design and fundamental R\&D efforts, since these two aspects of the
project are clearly not independent. The new project structure will be
in place by mid 2007.

The GDE remains committed to the technically-driven schedule of supplying the EDR in 2010, making start of construction possible as early as 2012 – consistent with expected early results from the LHC. The critical path and cost drivers have been clearly identified during the RDR phase, and they define the priorities for the next three years of the Engineering Design phase. The R\&D program will be fine-tuned to mitigate the remaining identified technical risks of the design. A key element of the engineering activity will be the formation of a qualified industrial base in each region for the SCRF linac technology. A equally critical focus will be on the civil construction and conventional facilities – the second primary cost driver – where an early site selection would clearly be advantageous.

Finally, the GDE also remains committed to completing these challenging goals as a truly international organization, by building on and consolidating the successful collaboration which produced the RDR. The support of the world-wide funding agencies is critical in this endeavor. The GDE – together with the leaders of the particle physics community – will continue to work with the regional funding agencies and governments to begin construction of this project in the early part of the next decade.


[BF1]I couldn't understand this sentence as it stood – I think this is what is meant.


==> orig/table3-2.tex <==
\begin{table}[hbt]
\begin{center}
\caption{Some key parameters of the four detector concepts.
\label{Detectors:concepts}}
\begin{tabular}{|l|c|c|c|c|c|c|}\hline%
Concept & Tracking & Solenoidal & Radius, & Rvtx & Recal & Rmax, \vspace{-6pt} \\%
 & Technology & Field & Length & (mm) & Lecal & $\frac{1}{2}$ L \vspace{-6pt} \\%
 & & (Tesla) & of & Rin TPC & (meters) & (meters) \vspace{-6pt} \\%
 & & & Solenoid & & & \vspace{-6pt} \\%
 & & & (meters) & & & \\ \hline  & & & & \vbdlspacing \hline%
GLD & TPC & 3 & 4.9,7 & 20 & 2.1 & 7.65 \\%
    &     &   &       &    & 2.8 & 8.0 \\ \hline%
LDC & TPC & 4 & 3,6.6 & 15.5 & 1.58 & 5.98 \\%
    &     &   &       &    & 2.3 & 5.60 \\ \hline%
SiD & Silicon & 5 & 2.5,5.5 & 14 & 1.27 & 6.45 \\%
    &         &   &         &    & 1.27 & 5.89 \\ \hline%
4$^{\rm th}$  & TPC & 3.5 & & & & \\ \hline%
\end{tabular}
\end{center}
\end{table}

